Near-Optimal Procedures for Model Discrimination with Non-Disclosure Properties

Let $\theta_0,\theta_1 \in \mathbb{R}^d$ be the population risk minimizers associated to some loss $\ell:\mathbb{R}^d\times \mathcal{Z}\to\mathbb{R}$ and two distributions $\mathbb{P}_0,\mathbb{P}_1$ on $\mathcal{Z}$. The models $\theta_0,\theta_1$ are unknown, and $\mathbb{P}_0,\mathbb{P}_1$ can be accessed by drawing i.i.d samples from them. Our work is motivated by the following model discrimination question: "What sizes of the samples from $\mathbb{P}_0$ and $\mathbb{P}_1$ allow to distinguish between the two hypotheses $\theta^*=\theta_0$ and $\theta^*=\theta_1$ for given $\theta^*\in\{\theta_0,\theta_1\}$?" Making the first steps towards answering it in full generality, we first consider the case of a well-specified linear model with squared loss. Here we provide matching upper and lower bounds on the sample complexity as given by $\min\{1/\Delta^2,\sqrt{r}/\Delta\}$ up to a constant factor; here $\Delta$ is a measure of separation between $\mathbb{P}_0$ and $\mathbb{P}_1$ and $r$ is the rank of the design covariance matrix. We then extend this result in two directions: (i) for general parametric models in asymptotic regime; (ii) for generalized linear models in small samples ($n\le r$) under weak moment assumptions. In both cases we derive sample complexity bounds of a similar form while allowing for model misspecification. In fact, our testing procedures only access $\theta^*$ via a certain functional of empirical risk. In addition, the number of observations that allows us to reach statistical confidence does not allow to "resolve" the two models $-$ that is, recover $\theta_0,\theta_1$ up to $O(\Delta)$ prediction accuracy. These two properties allow to use our framework in applied tasks where one would like to $\textit{identify}$ a prediction model, which can be proprietary, while guaranteeing that the model cannot be actually $\textit{inferred}$ by the identifying agent.

==> apx-plug.tex <==
\section{Asymptotic bound for test~\eqref{eq:test_plug-in}}
\label{app:plug}

We assume that~$r_0 = r_1 = r$ for simplicity.
Our goal is to show that, in the asymptotic regime~$n \to \infty$ with fixed~$r$ and~$\Delta_0, \Delta_1$, the type I error of the plug-in test~\eqref{eq:test_plug-in} satisfies 
\[
\Prob_{\cH_0}[\wh T = 1] \to P_{\infty} \le C \exp(-cn[\Delta_0 + \Delta_1]). 
\]
Now, from step~\proofstep{2} of the proof of Theorem~\ref{th:lower-gaussian}, more precisely~\eqref{eq:lower-easy}, we recall that the type-I error of~$\wh T_{LR}$ (cf.~\eqref{eq:test-oracle-sims}) writes
\begin{equation}
\label{eq:plug-in-comparison}
\Prob_{\cH_0}[\wh T_{LR} = 1] = \Prob[\wh S \ge 0] 
= \Prob\big[\wh W \ge n[\Delta_0 + \Delta_1]\big] 
\le C\exp(-cn[\Delta_0 + \Delta_1]),
\end{equation}
where~$\wh S$ is the statistic whose sign is examined by~$\wh T_{LR}$, and~$\wh W$ is the centering of~$\wh S$.  
The final inequality here is ``robust'' to~$\Delta_1$ (i.e., allows to change~$\Delta_1$ by a constant factor). Thus, defining
\[
\begin{aligned}
\wh E_0 &= \| Y - X (\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 - \| Y - X \bar\theta\|^2, \\
\wh E_1 &= \| \wt Y - \wt X (\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 - \| \wt Y - \wt X \bar\theta\|^2, \\
\end{aligned}
\]
we have that
\[
\begin{aligned}
\Prob_{\cH_0}[\wh T = 1] 
&= 
\Prob \big[\wh W - \wh E_0 + \wh E_1  \ge n[\Delta_0 + \Delta_1] \big] \\
&\le
\Prob [\wh E_1 - \wh E_0 \ge n[\Delta_0 + \Delta_1]/2 + \Prob \big[\wh W \ge n[\Delta_0 + \Delta_1]/2\big]\\ 
&\le 
\Prob [\wh E_1 - \wh E_0 \ge n\Delta_0/2] + C\exp(-n[\Delta_0 + \Delta_1]),
\end{aligned}
\]
where in the last step we used~\eqref{eq:plug-in-comparison}.
It remains to bound the deviations for~$\wh E_0$ and~$\wh E_1$. 

Now, recall that~$\theta^* = \theta_0$ and~$\bar\theta = \theta_1$ under~$\cH_0$. Denoting~$\wh \delta_k = \wh\theta_k - \theta_k$ for~$k \in \{0,1\}$, we have
\[
\begin{aligned}
\wh E_0 &= \|X(\wh\delta_0 + \wh\delta_1)\|^2 - 2\langle X (\wh \delta_0 + \wh \delta_1), X^\top \xi + X(\theta_1 - \theta_0) \rangle, \\
\wh E_1 &= \|\wt X(\wh\delta_0 + \wh\delta_1)\|^2 - 2\langle \wt X (\wh \delta_0 + \wh \delta_1), \wt X^\top \wt \xi \rangle.
\end{aligned}
\]
Now, assume for simplicity (this holds in our experimental setup in Sec.~\ref{sec:simul}) that~$X, \wt X$ have the same covariance matrix~$\bSigma$ with rank~$r$. Observe that, when~$n \to $
\qed

==> apx-remainder.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Remaining proofs}
\label{app:aux}
  

  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Consider the case where~$\rank(X)=\rank(\tilde{X}) = r$, $\lambda_{\min}(XX^{\top}) = \lambda_{\min}(\tilde{X}\tilde{X}^{\top}) = 1/\kappa$ for some $\kappa>1$ and the other non-zero eigenvalues equal to $\kappa>1$. We choose~$\tilde{X}(\theta_1 - \theta_0)$  to be the eigenvector corresponding to $\lambda_{\min}(\tilde{X}\tilde{X}^{\top})$ and assume that 
%\[
%\|\tilde{X}(\theta_0 - \theta_1)\|^2 \leq \|X(\theta_0 - \theta_1)\|^2.
%\]
%Hence 
%\[
%\Prob_0[\hat{T} = 1|X,\tilde{X}] + \Prob_1[\hat{T} = 0|X,\tilde{X}] \le C \exp (-c  \|\tilde{X}(\theta_0-\theta_1)\|^2 \min[1, \|\tilde{X}(\theta_0-\theta_1)\|^2/\bar r]).
%\]
%On the other hand, we have 
%\[
%\Prob_{0}[\hat{T}_g = 1 | X,\tilde{X}] 
%= \Prob \big[ \| X^{\top}\xi\|^2 - \|\wt X^\top \wt \xi\|^2 + 2\langle \tilde{X}(\theta_1 - \theta_0),\tilde{X}^\top\tilde{\xi} \rangle \geq \| \wt X(\theta_1 - \theta_0)\|^2/\kappa \big] .
%%\| \tilde{X}(\theta_0 - \theta_1)\|^2
%\]
%By rotation invariance we can write $\|X^\top\xi\|^2$ as $\zeta_r^2/\kappa + \sum_{i=1}^{r-1}\zeta_i^2$, where $\zeta_i$ are i.i.d standard random Gaussian variables. We also have that 
%\[
%\sqrt{\Var\left( \underbrace{\zeta_r^2/\kappa - \|\wt X^\top \wt \xi\|^2 + 2\langle \tilde{X}(\theta_1 - \theta_0),\tilde{X}^\top\tilde{\xi} \rangle}_{Z} \right)} \leq  2\sqrt{r} + 2\|\tilde{X}(\theta_1 - \theta_0)\|/\sqrt{\kappa}.
%\]
%Observing that
%\[ 
%\Prob_0(\mathcal A) := \Prob_0\left[ Z \leq \E Z + 2 \sqrt{\Var(Z)}  \right] \geq 1/2.
%\]
%Hence as long as $\|\tilde{X}(\theta_1 - \theta_0)\|^2 \geq  \sqrt{r}\kappa $, we have 
%\[ 
%\Prob_{0}[\hat{T}_g = 1 | X,\tilde{X}]  \geq 0.5\Prob \left[ \sum_{i=1}^{r-1}(\zeta_i^2-1) \geq 9\|\tilde{X}(\theta_1 - \theta_0)\|^2/\kappa  \right].
%\]
%We conclude using a lower bound on the chi-square tail \eqref{eq:tail_square} that
%\[
%\Prob_{0}[\hat{T}_g = 1 | X,\tilde{X}]  \geq C \exp (-c  \|\tilde{X}(\theta_0-\theta_1)\|^4/(\kappa^2\bar r)].
%\]
%It turns out that as $\kappa$ grows, then test $\hat{T}_g$ can have an exponentially larger error compared to $\hat{T}$ in the regime $  \sqrt{r}\kappa \leq \|\tilde{X}(\theta_1 - \theta_0)\|^2 \leq r\kappa$. Hence $\hat{T}_g$ is sub-optimal in a minimax sense.



%\section{\odima{to pass} Adaptive testing for linear model}
%\label{app:adaptive}
%For simplicity let~$n_0 = n_1 = n$ and assume that~$\wh \bSigma_0, \wh \bSigma_1$ are both full-rank. 
%In the well-specified linear model, and when the noise variances $\sigma_0^2,\sigma_1^2$ are known, test \eqref{eq:test_1} is given by
%\[
%\hat{T} = \ind\left\{ \| Y - X\theta^*\|^2_X - \sigma_0^2\rank(\wh \bSigma_0) \geq \| \tilde{Y} - \tilde{X}\theta^* \|^2_{\tilde{X} } - \sigma_1^2\rank(\wh \bSigma_1) \right\},
%\]
%where $\sigma_0^2 , \sigma_1^2$ are respectively variances of $Y-X\theta_0$ and $\tilde{Y} - \tilde{X}\theta_1$. In order to make our test adaptive to noise, we start by estimating $\sigma$ (and in the same way $\tilde{\sigma}$). Recall that
%$$
%Y = X\theta_0 + \sigma_0 \varepsilon,
%$$
%where $\varepsilon$ is the standard Gaussian vector. We consider two estimators of $\sigma_0^2$ depending on $\rank(\wh \bSigma_0)$. 
%\begin{itemize}
%    \item  $\rank(\wh \bSigma_0) \leq n/2$:
%    
%In this case, we define 
%$$
%\wh \sigma_0^2 := \frac{\| Y - X\theta^*\|^2_{X^c}}{n- \rank(\wh \bSigma_0) },
%$$
%where $\|.\|_{X^c}$ corresponds to the norm of the projected vector on the space orthogonal to span($X$). It follows that, for all $t \geq 0$, we have
%$$
%\Prob( |\wh \sigma_0^2 / \sigma_0^2 -1 | \geq t) \leq e^{-cn(t^2\wedge t )}.
%$$
%
%\item $\rank(\wh \bSigma_0)  \geq n/2$:
%
%In this case, we sample two identical copies of $(X,Y)$ given by $(X_1,Y_1)$ and $(X_2,Y_2)$ and define 
%$$
%\wh \sigma_0^2 := \frac{\left\|\left( (X_1^{\top}X_1)^{-1} + (X_2^{\top}X_2)^{-1} \right)^{-1/2}\left((X_1^{\top}X_1)^{-1}X_1^{\top}Y_1- (X_2^{\top}X_2)^{-1}X_2^{\top} Y_2\right)\right\|^2}{\rank((X_1^{\top}X_1)^{-1} + (X_2^{\top}X_2)^{-1})}.
%$$
%One may observe that $\sigma_2^2 \sim \sigma^2 \chi_r^2 / r$ where $r=\rank((X_1^{\top}X_1)^{-1} + (X_2^{\top}X_2)^{-1})$.
%Hence we get that, for all $t \geq 0$
%\[
%\Prob( |\wh \sigma_0^2 / \sigma_0^2 -1 | \geq t) \leq e^{-cn(t^2\wedge t)},
%\]
%since $r\geq n/2$.
%\end{itemize}
%
% In both cases the estimator $\hat{\sigma}^2$ satisfies for all $t \geq 0$
%\[
%\Prob[ |\hat{\sigma}_0^2 / \sigma_0^2 -1 | \geq t] \leq e^{-cn(t^2\wedge t)},
%\]
%and similarly for $\hat{\sigma}_1^2 $ corresponding to $(\tilde{X},\tilde{Y})$.
%We define the adaptive test $\tilde{T}$ such that
%\[
%\tilde{T} = \ind\left\{ \| Y - X\theta^*\|^2_X - \wh \sigma_0^2\wh r_0 \geq \| \tilde{Y} - \tilde{X}\theta^* \|^2_{\tilde{X} } - \wh \sigma_1^2\wh r_1 \right\},
%\]
%We can now show that estimation of the noise parameter does not impact the non adaptive rate. Let us denote by $\sigma^2:= \sigma_0^2 \vee \sigma_1^2 $.
%Following the proof of Proposition \ref{prop:upper-fixed-design}, we have
%\begin{align*}
%\Prob_{0}[\wt T = 1 | X, \tilde{X}] 
%&= \Prob \big[ \| \xi\|^2_X - \wh \sigma_0^2\wh r_0  
%	+ \wh \sigma_1^2\wh r_1 - \| \wt \xi\|^2_{\wt X} + 2\langle \tilde{X}(\theta_1 - \theta_0),\tilde{\xi} \rangle \geq n\wh \Delta_1^2 \big]  \\ 
%&\leq C\exp\big(-c n\wh \Delta^2/\sigma^2\min[1,  n\wh\Delta^2/(\wh r\sigma^2)]\big) 
%	+ 2\Prob\left[ |\hat{\sigma}_0^2 / \sigma_0^2 -1 | \geq \frac{n\wh \Delta^2}{3\sigma^2 \hat{r}} \right] \\
%& \leq C\exp\big(-c n\wh \Delta^2/\sigma^2\min[1,  n\wh\Delta^2/(\wh r\sigma^2)]\big) 
%	+ 2\exp\big(-c n^2\wh \Delta^2/(\sigma^2\wh r)\min[1,  n\wh\Delta^2/(\wh r\sigma^2)\big)
%\\
%& \leq C'\exp\big(-c' n\wh \Delta^2/\sigma^2\min[1,  n\wh\Delta^2/(\wh r\sigma^2)]\big),
%\end{align*}
%where the last inequality holds since $\hat{r} \leq n$. 
%\normalsize

==> extra/preamble.tex <==
%     \usepackage[preprint]{neurips_2020}
%     \usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{amsmath, amsfonts, amssymb, amsthm}
%\usepackage{color}
%\usepackage{url}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{subfigure}
\usepackage{paralist}

\usepackage{comment}

\usepackage{mathrsfs}

\usepackage{fullpage}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\definecolor{darkgreen}{rgb}{0.0,0,0.9}
\usepackage[pagebackref,colorlinks=true,pdfpagemode=none,citecolor=OliveGreen,linkcolor=BrickRed,urlcolor=BrickRed,pdfstartview=FitH]{hyperref}
\usepackage{color}
%\usepackage{showkeys}


\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{proposition*}{Proposition}
\newtheorem*{corollary*}{Corollary}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{note}{Note}
\newtheorem*{note*}{Note}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem*{definition*}{Definition}


%%%%%%%%%%%%%%%%%% DIMA MACROES %%%%%%%%%%%%%%%%%%%
\usepackage{xcolor}
\usepackage{dsfont}
\newcommand{\odima}[1]{{\color{violet}#1}}
\newcommand{\simo}[1]{{\color{red}#1}}
\newcommand{\adel}[1]{{\color{blue}#1}}
\newcommand{\meisam}[1]{{\color{green}#1}}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\R}{\mathds{R}}
\newcommand{\E}{\mathds{E}}
\newcommand{\Prob}{\mathds{P}}
\newcommand{\lsim}{\lesssim}
\newcommand{\gsim}{\gtrsim}
\newcommand{\rank}{\textup{rank}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\sign}{\textup{sign}}
\newcommand{\lang}{\left\langle}
\newcommand{\rang}{\right\rangle}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cD}{\mathds{D}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\G}{\boldsymbol{G}}
\renewcommand{\H}{\boldsymbol{H}}
\newcommand{\T}{\boldsymbol{T}}
\newcommand{\M}{\boldsymbol{J}}
\newcommand{\Mopt}{\M^{\boldsymbol\star}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\Id}{\boldsymbol{I}}
\newcommand{\weakto}{\rightsquigarrow}
\newcommand{\Tr}{\textup{Tr}}
\newcommand{\proofstep}[1]{$\boldsymbol{{#1}^o}$}
\newcommand{\Var}{\textup{Var}}
\newcommand{\Bias}{\textsf{\textup{b}}}
\renewcommand{\tilde}{\wt}
\renewcommand{\hat}{\wh}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\Argmin}{Argmin}
\newcommand{\tht}{\theta}
\newcommand{\rmin}{\texttt{r}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\piC}{\pi_{\cC}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\renewcommand{\le}{\leq}
\renewcommand{\ge}{\geq}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\newcommand{\pinv}{\dagger}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}

\newcommand{\ue}{\textup{e}}

\newcommand{\learner}{\textit{Learner}}
\newcommand{\auditor}{\textit{Auditor}}

\newcommand{\Cov}{\textup{Cov}}

\newcommand{\cT}{\textsf{T}}

\newcommand{\lp}{\vspace{0.1cm}\vspace{-0.1cm}'}
\newcommand{\lpp}{\vspace{0.1cm}\vspace{-0.1cm}''}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHORS INFO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.
\if false
\author{%
  Author\thanks{Use footnote for providing further information
    about author (webpage, alternative address)---\emph{not} for acknowledging
    funding agencies.} \\
  Department of ....\\
  University of Southern California\\
  Los Angeles, LA 90007 \\
  \texttt{author1@usc.edu} \\
  % examples of more authors
   \And
   Coauthor \\
   Department of ....\\
   University of Southern California \\
  Los Angeles, LA 90007 \\
   \texttt{author2@usc.edu} \\
  % \AND
   \And
   Adel Javanmard \\
   Marshall School of Business\\
   University of Southern California \\
  Los Angeles, LA 90007 \\
   \texttt{author3@usc.edu} \\
  % \AND
  \And
   Adel J \\
   Department of ....\\
   University of Southern California \\
  Los Angeles, LA 90007 \\
   \texttt{author4@usc.edu} \\
  % \AND
}
\fi

==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}

%In recent years, theoretical and practical advances in the field of  have revolutionized a wide range of engineering and scientific disciplines. However, this rapid growth poses significant societal risks such as potential for unfair/discriminatory outcomes and violating individuals' privacy. 

Statistical learning theory has seen tremendous progress in the past decades and revolutionized a wide range of engineering and scientific disciplines in its turn (see, e.g.,~\cite{shalev2014understanding,hastie2009elements,bousquet2003introduction} and references therein).
Speaking informally, its main goal is constructing prediction models that generalize, i.e., have statistical performance guarantees on previously unseen examples.
Taking a frequentist point of view, this can be conveniently formalized in the language of~$M$-estimation~(\cite{lehmann2006theory,borovkov,van2000asymptotic}):
one identifies possible ``models'' in a given learning task with~$\theta \in \R^d$, and models ``previously unseen example'' as a random observation~$z$ from some space~$\cZ$.
The performance of a candidate model~$\theta$ on a specific example~$z$ can then be measured through some {loss function}~$\ell_z: \R^d \to \R$. 
Learner's task is then to approximately minimize {\em the population risk}~$L(\theta) := \E_{z \sim \Prob}[\ell_z(\theta)]$, where the expectation is over the unknown distribution~$\Prob$ of~$z$, by observing a random i.i.d.~sample~$z_1, ..., z_n \sim \Prob$. A very natural, and arguably the most commonly used approach to solving this task amounts to minimizing, instead of~$L(\theta)$, the {\em empirical risk}
$
\wh L(\theta) := \frac{1}{n} \sum_{i = 1}^{n} \ell_{z_i}(\theta).
$
%and minimizing~$\wh L(\theta)$ in place of~$L(\theta)$. 
Since~$\wh L(\theta)$ is an unbiased estimate of~$L(\theta)$, one can usually prove convergence of the obtained {empirical risk minimizer}~$\wh \theta$ to a minimizer of~$L(\theta)$, e.g., via some uniform version of the law of large numbers. 
The quantitative aspect consists in establishing the rate of this convergence. 
\odima{More precisely, rather than estimating the target population risk minimizer~$\theta^*$, one is often more interested in the prediction performance of~$\wh\theta$ in terms of {\em excess risk}~$L(\wh \theta) - \min_{\theta \in \Theta} L(\theta)$, where~$\Theta \subseteq \R^d$ is a parametric set. The differences between estimation and prediction, however,  the error is measured by the ``prediction'' distance linked to the local quadratic expansion of~$L(\theta)$ at~$\theta^*$~(\cite{Lecam1975,Lecam1986,spokoiny2012parametric,ostrovskii2018finite}), 
and we do not distinguish between these two tasks later on.} %in what follows.
%Moreover, it is oftentimes of little interest how well~$\wh\theta$ estimates the population risk minimizer; rather, one is interested in the prediction performance of~$\wh\theta$ in terms of {\em excess risk}~$L(\wh \theta) - \min_{\theta} L(\theta)$.

One conventional wisdom in statistics is that testing is easier than estimation. 
For example, reductions to testing problems are often used when proving minimax lower bounds in parametric estimation problems~\cite{tsybakov_mono,nemirovski2000topics}.
This is done by first lower-bounding the minimax risk in terms of the testing error in a derived hypothesis testing problem, and then characterizing this testing error using information-theoretic arguments or even deriving it exactly.
However, in this application one rarely encounters the situations where testing is {\em qualitatively} easier than estimation, rather than ``just as hard''.
Such situations do arise -- most notably, in detection-type problems, where one would like to detect the presence of a signal in noisy observations. 
Signal detection can be easier than estimation, for example, because the former task may not require localizing the signal or estimating its direction, and thus does not have to deal with the complexity of the whole space of hypotheses.
Along these lines, statistical and computational gaps between signal detection and estimation have been observed, e.g., in sparse linear regression~\cite{donoho2016high,ingster2010detection} and in the spiked covariance model~\cite{berthet2013optimal}.\\

In this paper, we introduce a novel testing problem which is qualitatively easier than the associated estimation problem.
Rather than being of a ``signal detection'' kind, this testing problem has a more classical flavor of distinguishing between two ``peer'' hypotheses about the data distribution. 
Prior to formulating it, let us look at a couple of motivating examples.

\paragraph{Example 1.}
Given~$\mu_0,\mu_1 \in \R^d$, consider distinguishing between the two hypotheses~$\cH_0: \mu^* = \mu_0$ and~$\cH_1: \mu^* = \mu_1$ in the Gaussian mean model, i.e., by observing the i.i.d.~copies~$z_1, ..., z_n$ of
%about the mean of a shifted~$d$-dimensional standard Gaussian vector
\[
z = \mu^* + \xi \sim \cN(\mu^*,\Id_d).
\]%Since we are in the situation of two simple hypotheses, by the Neyman-Pearson lemma~(\cite{lehmann2006testing}) the likelihood-ratio test.
A very natural approach is to estimate~$\mu^*$ via the sample average~$\wh \mu$ and choose the closest to~$\wh \mu$ point among~$\{\mu_0, \mu_1\}$. 
Note that this is equivalent to averaging observations first projected along~$\mu_1-\mu_0$, and leads to noise reduction -- removal of the component of~$\xi$ orthogonal to~$\mu_1-\mu_0$.
The {\em sample complexity} of this test, defined as the sample size necessary and sufficient to guarantee fixed error probabilities of both types (say, at most 0.05), is~$O(1/\Delta)$, where~$\Delta$ is the squared Euclidean distance between~$\mu_0$ and~$\mu_1$.\footnote{Later on,~$O(\cdot)$ and~$\Omega(\cdot)$ hide a constant factor;~$\|\cdot\|$ is the~$\ell_2$-norm for vectors and the operator norm for matrices.}
Moreover, by the Neyman-Pearson lemma~\cite{lehmann2006testing} this bound is sharp, and the test is optimal with respect to the risk given by the sum of error probabilities.
Meanwhile, {\em estimating}~$\mu^*$ up to~$O(\sqrt{\Delta})$ error (i.e., with accuracy matching the ``scale'' of the testing problem) requires~$\Omega(d/\Delta)$ observations, compared to~$O(1/\Delta)$ for testing.
%In this sense, estimation is indeed harder than testing here.

\paragraph{Example 2.}
In the previous example, the testing problem is easy because a single direction is relevant for it, and this direction is known to the statistician.
But what if the direction is unknown? 
Let us change the problem setup: now we assume that~$\mu^*$ is known, but~$\mu_0$ and~$\mu_1$ {\em are not}. Formally, the two hypotheses to test are the same as before (i.e.,~$\cH_0: \mu^* = \mu_0$ against~$\cH_1: \mu^* = \mu_1$), but this time we are granted two i.i.d.~samples~$z_1, ..., z_{n}$ and~~$\wt z_1, ..., \wt z_{n}$ generated according to~$\cH_0$ and~$\cH_1$ correspondingly, i.e., with means~$\mu_0$ and~$\mu_1$. 
A very natural approach in this situation is to compare the distances between~$\mu^*$ and the two sample average estimates~$\wh \mu_0$ and~$\wh \mu_1$, i.e., apply the test
%\footnote{Here and in what follows, we always use the~$\ell_2$-norm for vectors and operator norm for matrices.}
\begin{equation}
\label{eq:shift-test}
\wh T = 
\ind \left\{ \|\wh \mu_0 - \mu^*\|^2 - \|\wh \mu_1 - \mu^*\|^2 \ge 0\right\}.
\end{equation}
% Using the standard chi-square and Gaussian tail bounds, 
We can easily verify that the sample complexity of this test, in the same sense as before, is~$O(\sqrt{d}/\Delta)$. 
Indeed, since~$\zeta := \sqrt{n}(\wh \mu_0 - \mu_0)$ and~$\wt \zeta := \sqrt{n}(\wh \mu_1 - \mu_1)$, are independent and distributed as~$\cN(0,\Id_d)$, we can bound the type I error probability as follows:
\begin{align}
\Prob_{\cH_0}[\wh T = 1] 
&= 
\Prob \big[ \|\wh \mu_0 - \mu_0\|^2 - \|\wh \mu_1 - \mu_1 + \mu_1 - \mu_0\|^2 \ge 0 \big] \notag\\
&= 
\Prob \big[ \|\zeta\|^2 - \|\wt \zeta \|^2 + 2\sqrt{n}\langle \wt\zeta, \mu_0 - \mu_1 \rangle \ge n\Delta \big] \notag\\
&\le
\Prob \big[ \|\zeta\|^2 - d \ge n\Delta/3 \big] + \Prob \big[ d - \|\wt \zeta \|^2 \ge n\Delta/3 \big] + \Prob \big[ 2\sqrt{n}\langle \wt\zeta, \mu_0 - \mu_1 \rangle \ge n\Delta/3 \big].
\label{eq:shift-error-decomposition}
\end{align}
Since~$\|\zeta\|^2, \|\wt \zeta\|^2 \sim \chi_d^2$ and~$\langle \wt\zeta, \mu_0 - \mu_1 \rangle \sim \cN(0,\Delta)$, applying the standard chi-square and Gaussian tail bounds (see, e.g.,~\cite[Lemma~1]{laurent2000adaptive}), we bound the right-hand side as~$O(\max[e^{-cn^2\Delta^2/d},e^{-cn\Delta}])$ for some~$c > 0$, and similarly for the type II error by symmetry.
This corresponds to~$O(\sqrt{d}/\Delta)$ sample complexity.
While this sample complexity now depends on~$d$, here again testing is, in a sense, easier than estimation: the deviation of~$\wh \mu_0$ (resp.,~$\wh \mu_1$) from~$\mu_0$ (resp.,~$\mu_1$) is of order~$\sqrt{d/n}$, thus the sample size to guarantee~$O(\sqrt{\Delta})$ deviation is of order~$d/\Delta \; [\gg \sqrt{d}/\Delta]$.
%Yet, the sample complexity of testing is not dimension-independent anymore. 
%
In fact,~\eqref{eq:shift-error-decomposition} shows that one part of the error probability comes from the cross-term, in which observations are projected to the direction~$\mu_1-\mu_0$ as in the first example. 
Hence, we are as well solving the underlying Gaussian mean testing problem along a given direction, for which the sample complexity is~$O(1/\Delta)$. 
However, now we pay for the direction being unknown: the dominating part of the error probability now comes from the quadratic term~$\|\zeta\|^2-\|\wt \zeta\|^2$, resulting in sample complexity~$O(\sqrt{d}/\Delta)$. 
% as if the direction was known -- and is dominated already when~$n = c/\Delta$; thus, we are as well solving the underlying ``one-dimensional'' testing problem.   
%However, the dominating part of error probability now comes from the chi-squared terms, as in the estimation case.
On the other hand, here~$\|\zeta\|^2$ and~$\|\wt \zeta\|^2$ compensate each other on average, and the error is only due to their fluctuations around the common mean, which improves the sample complexity compared to the estimation case.
%This is precisely the mechanism behind the improvement of sample complexity compared to estimation. 

%\subsection{Problem formulation}
%\label{sec:setup}

\paragraph{Problem formulation.}
Our problem of interest is essentially an extension of the previous example to the general~$M$-estimation setup. 
More precisely, our task is to distinguish between the hypotheses 
\begin{equation}
\label{eq:hypotheses}
\cH_0: \{\theta^* = \theta_0 \}, \quad 
\cH_1: \{\theta^* = \theta_1 \},
\end{equation}
where~$\theta_0,\theta_1$ are the population risk minimizers for two candidate distributions~$\Prob_0, \Prob_1$ of~$z$, that is
\begin{equation}
\label{eq:minimizers}
\theta_k = \argmin_{\theta \in \R^d} \left\{ L_k(\tht) := \E_{z \sim \Prob_k} [\ell_z(\tht)] \right\} \quad (k \in \{0,1\}),
\end{equation}
and~$\theta^* \in \R^d$ is a given vector. The loss~$\ell_z: \R^d \to \R$ is assumed strictly convex in order to guarantee the uniqueness of~$\theta_0,\theta_1$.
To construct a test, statistician is granted access to the two i.i.d.~samples:
\begin{equation}
\label{eq:samples}
Z := (z_1, ..., z_{n_0}) \sim \Prob_0^{\otimes n_0}, \quad 
\wt Z := (\wt z_1, ..., \wt z_{n_1}) \sim \Prob_1^{\otimes n_1}.
\end{equation}
The performance of a test~$\wh T: (Z, \wt Z, \theta^*) \to \{0,1\}$ is measured by the largest of two error probabilities~$\Prob_{\cH_0}[\wh T=1], \Prob_{\cH_1}[\wh T=0]$. 
%the maximum over the error probabilities of both types: 
Thus, the associated sample complexity, which we aim to characterize, corresponds to the necessary and sufficient~$n_0,n_1$ to guarantee fixed error probabilities of both types (for example, at most 0.05). %and we aim at characterizing it (often assuming~$n_0 = n_1$ for simplicity) 
\odima{Specify what else is known.}

\paragraph{Practical motivation.}
% Although the above testing problem might seem somewhat artificial and not practically relevant, it arises in some 
A very important application of the above testing problem is in ``privacy-aware'' machine learning tasks (see Sec.~\ref{sec:applications} for more details).
In a nutshell, this is due to the fact that our proposed testing procedures in fact {\em  do not require direct access to~$\theta^*$}. 
Instead,~$\theta^*$ is accessed through a pair of {\em empirical prediction scores} -- two random measurements (in fact, real numbers) that evaluate how well~$\theta^*$ fits the two samples
Thus, these procedures can be run without communicating~$\theta^*$ to the testing agent. 
Furthermore, our derived bounds on sample complexity are {\em way smaller} than the sample complexity of {\em estimating}~$\theta_0,\theta_1$ up to accuracy~$O(1/\Delta)$, 
and thus also than the sample complexity of estimating~$\theta^*$ from the empirical prediction scores.\footnote{Indeed, the latter task amounts to estimating~$\theta_0,\theta_1$ and testing~$\cH_0$ against~$\cH_1$ to decide which of the two is~$\theta^*$.} 
Apart from illustrating the gap between testing and estimation, this gap guarantees {\em a degree of privacy} in applications where~$\theta^*$ is unknown.
We defer further discussion of applications framework to Sec.~\ref{sec:applications} in order to put them into the context of our results.


\paragraph{Notation.} 
We use~$C,c,c',c_1$, etc., for generic positive constants. 
We write~$g = O(f)$ (or~$f = \Omega(g)$) to state that~$g(t) \le Cf(t)$ uniformly over all possible values of~$t$.
Notation~$f \ll g$ (or~$g \gg f$) is the negation of~$g = O(f)$. We let~$a\vee b := \max(a,b)$ and~$a \wedge b := \min(a,b)$. We denote~$[n] := \{1, 2, ..., n\}$ for~$n \in \mathds{N}$. We use~$\| \cdot \|$ for the~$\ell_2$-norm of a vector and the largest eigenvalue of a positive-semidefinite (PSD) matrix. We use bold symbols for PSD matrices.
We denote~$\M^\dagger$ the generalized inverse of a PSD matrix~$\M$, i.e., the matrix with the same eigenbasis as~$\M$ and inverse non-zero eigenvalues, and let~$\M^{\dagger/2}$ be the PSD square root of~$\M^\dagger$. 
% in the case of matrices, the argument is always positive-semidefinite (PSD). 
We denote~$\|u\|_A := \|\bPi_{A} u\|^2$, where~$\bPi_A := A(A^{\top}A)^{\dagger}A^{\top}$ is the projector onto the column space of matrix~$A$. 
We denote~$\Id_r$ the~$r \times r$ identity matrix. 
We use the ``Matlab notation'' for matrix concatenation:~$[A,B]$ and~$[A;B]$ denote, correspondingly, the horizontal and vertical concatenation of two matrices with compatible dimensions.
%We defer the proofs to appendix.


\subsection{Overview of ideas, contributions and paper organization}
\label{sec:contrib}

We make important first steps towards solving the general case of the problem given in Eqs.~\eqref{eq:hypotheses}--\eqref{eq:samples}.
% as formulated above.

In Sec.~\ref{sec:gaussian}, we focus on the case of well-specified linear regression with random design, where we have an almost complete picture. 
Here we assume that~$z = (x,y)$ with~$x \in \R^d$ and~$y \in \R$, and assume the distributions~$\Prob_0, \Prob_1$ to be Gaussian, namely,
%We specify the two distributions~$\Prob_{0}$ and~$\Prob_1$ of the pair~$(x,y)$ as follows:
\[
\begin{aligned}
%\Prob_0: x \sim \cN(0,\bSigma_0), \; y|x &\sim \cN(x^\top \theta_{0},1),\\ 
%\Prob_1: x \sim \cN(0,\bSigma_1), \; y|x &\sim \cN(x^\top \theta_{1},1), 
\Prob_k: x \sim \cN(0,\bSigma_k), \; y|x &\sim \cN(x^\top \theta_{k}^{\vphantom 2},\sigma_k^2) \quad (k \in \{0,1\}).
\end{aligned}
\]
We first assume the noise variances to be known, which is equivalent to~$\sigma_0^2 = \sigma_1^2 = 1$ by rescaling; however, other parameters $\theta_0,\theta_1,\bSigma_0,\bSigma_1$ are assumed unknown. 
Writing the two samples~\eqref{eq:samples} in a concise form as~$(X,Y)$ and~$(\wt X, \wt Y)$ with~$X \in \R^{n_0 \times d},\wt X \in \R^{n_1 \times d},Y\in \R^{n_0},\wt Y \in \R^{n_1}$, our proposed test is based on the high-level idea of comparing the magnitude of residuals at~$\theta^*$ for the two samples, that is~$\|Y - X \theta^*\|^2$ and~$\|\wt Y - \wt X \theta^*\|^2$. Yet, in order to work, this idea requires certain modifications. 
\begin{itemize}
\item%[--]
First, instead of using with the residuals directly, we first project them onto the respective signal spaces -- the column spaces of~$X$ and~$\wt X$. 
\item%[--]
Second, instead of comparing the squared norms of projected residuals, we compare their {\em fluctuations} from the mean under the referent hypothesis, using that these means are known.
\end{itemize}
When combined together, these two tricks result in a test with the sample complexity upper bound
\begin{equation}
\label{eq:intro-complexity}
O\bigg(\min\bigg[\frac{1}{\Delta^2}, \frac{\sqrt{r_0 \vee r_1}}{\Delta} \bigg] \bigg),
\end{equation}
where~$r_k = \rank(\bSigma_k)$ and~$\Delta = \min_{k \in \{0,1\}}[\|\bSigma_k^{1/2}(\theta_1 - \theta_0)\|^2]$ is the smaller prediction distance.
In this complexity estimate, the second bound essentially corresponds to the Gaussian shift scenario, except replacing the ambient dimension~$d$ with~$\max[r_0, r_1] \le d$. 
However, introducing projection allows to additionally exploit the presence of random design, leading to extra noise reduction, and results in the dimension-independent bound~$O(1/\Delta^2)$ that activates when~$\Delta \ge 1/\sqrt{\max[r_0, r_1]}$. 
We then show that the bound~\eqref{eq:intro-complexity} is nearly tight (up to the replacement of~$\max[r_0,r_1]$ with~$\min[r_0, r_1]$) by providing a minimax lower bound. 
Finally, we consider the case of unknown noise variances~$\sigma_0^2 \ne \sigma_1^2$, and construct an adaptive test that performs essentially the same as if these variances were known.
%One of them uses a non-standard technique for estimating the noise variances which allows to extend the approach beyond the case of linear model. 


In Sec.~\ref{sec:asymp}, we revisit the general~$M$-estimation setup.
Here we generalize the test from the linear regression scenario, replacing the squared norms of projected residuals with {\em empirical prediction scores}. 
These are defined as the Newton decrements~\cite{nesterov2013introductory} of empirical risks~$\wh L_0(\theta^*), \wh L_1(\theta^*)$ over the two samples. 
While the lower bound from the Gaussian case remains valid, deriving a general upper bound proves to be challenging. 
Hence, we focus on the asymptotic regime of large sample size and small separation with~$n\Delta \to \lambda$, in which the local Gaussian approximation applies~\cite{Lecam1986}.
%, namely~$n \to \infty$ and~$\Delta \to 0$ with~$n\Delta \to \lambda$, where~$\lambda > 0$ quantifies the complexity of the testing problem instead of the sample size. %($k \in \{0,1\}$). 
In terms of the derived dependency of the testing risk from~$\lambda$, the obtained results nearly match those in the Gaussian case, but also take into account the effect of model misspecification.
Finally, we show that the second-order information plays a {\em vital role}: the risk for a natural test in which one measures the gradients of empirical risks without using their Hessians can be {arbitrarily} larger than for our test.
%(indicating that well-specified parametric models behave as their Gaussian approximations), 
%the sample complexity bound~\eqref{eq:intro-complexity} for the Gaussian case, 
%For misspecified modes, the result is essentially preserved, except that the ranks~$r_0, r_1$ get replaced with the {\em effective ranks} that account for model misspecification. 


%\simo{emphasize adaptation in the asymptotic regime.}
%\odima{done later, I don't think we should put it here...}

In Sec.~\ref{sec:glm}, we extend our theory in another direction, now focusing on the {\em small-sample regime} 
\vspace{-0.1cm}
\[
%\label{eq:small-sample-regime-intro}
n \le \min[r_0,r_1].
\]
While estimation is clearly impossible in this regime (unless~$\Delta \gg 1$), the testing problem is still well-posed: according to~\eqref{eq:intro-complexity}, the sample complexity  falls in the above range unless~$\Delta$ is very small. %Hence, the small-sample regime is of main practical interest in the finite-sample scenario. 
Complementing our results for the Gaussian case, we consider generalized linear models (GLMs) in this regime. We again use a Newton-decrement based statistic, and prove an analogue of the bound~\eqref{eq:intro-complexity} under weak moment assumptions and moderate level of misspecification. As a byproduct, we extend the results of Sec.~\ref{sec:gaussian} to linear models with heavy-tailed noise.
From a technical viewpoint, small sample size leads to the diagonalization of the Newton decrements, with two advantages as the result: simpler statistical analysis and faster computation of the test statistic. 
%The advantage of this is twofold: simpler statistical analysis and faster computation of the test statistic. 

%In addition to simplifications in the analysis due to the explicit Newton decrements as the underlying projection becomes explicit; this also simplifies computation of the test statistic.
%\simo{+ we generalize linear regression result to heavy-tailed case as a consequence...}

In Sec.~\ref{sec:simul}, we present preliminary numerical experiments on synthetic data. We apply the framework to the task of the arbitrage of ``the right to be forgotten'' as explained in Sec.~\ref{sec:applications} below. The results of these experiments make a case for the practical relevance of our framework.
%, in which one of the distributions is modeled as a mixture. 
%While our sample complexity estimates might not be tight in this scenario, the proposed testing procedures can still be applied, and yield satisfactory results in practice. 

Next we discuss possible applications of our testing framework in privacy-aware machine learning.
 
%Thus, the proposed test only accesses~$\theta^*, Z, \wt Z$ through a local {second-order oracle} access to the empirical risk


 
%where~$\varepsilon \sim \cN(0,1)$ in both cases, 
%and let~$(X,Y)$,~$(\wt X, \wt Y)$ be i.i.d.~samples from ~$\Prob_0$ and~$\Prob_1$ respectively, with sizes~$n_0$ and~$n_1$.
%quadratic loss~$\ell_z(\theta) = \|y - x^\top \theta\|^2$, and 
%We begin from the analysis of a well-specified linear model 





%in the field of  have revolutionized a wide range of engineering and scientific disciplines. However, this rapid growth poses significant societal risks such as potential for unfair/discriminatory outcomes and violating individuals' privacy. 

%To control such adverse impacts, governments and consumer protection agencies have established guidelines and regulations, such as \cite{GDPR1,GDPR2,CCPA, FTC}, for organizations using AI. 
%While these guidelines seem  necessary to limit the potential adverse impact of AI, it is still not clear how to test for potential violations of these guidelines.
%As a first step towards building tools for this task, we develop a hypothesis testing procedure that verifies the type of data used in the training of a statistical model. Before describing our framework and results in detail, we briefly summarize the problem statement.





\subsection{Practical applications}
\label{sec:applications}

%\odima{{\bf TODO:} rewrite, extend, polish, add user identification, and possibly some other application?}

\paragraph{Arbitrage for ``the right to be forgotten.''}

% \noindent\textbf{Brief Problem Description.}  A \learner claims that she used a dataset $\mathcal{Z}$ (which can also be explained by probability distribution $P_Z$) to train her model $\mathcal{M}$. An \auditor suspects that the learner used the dataset~$\mathcal{\tilde{Z}}$ (which can also be explained by probability distribution $P_{\tilde{Z}}$) instead of dataset $\mathcal{Z}$. Assume the \auditor has minimal access to model $\mathcal{M}$ (as a blackbox) and has a number of samples from both distributions $P_{Z}$   and $P_{\tilde{Z}}$. Our question of interest is as follows: Can the \auditor test whether dataset $\mathcal{Z}$ is used in training or dataset $\mathcal{\tilde{Z}}$? 

Ubiquitous collection and storage of large volumes of user data by internet corporations poses societal risks such as potential for unfair/discriminatory outcomes and privacy violations.
To confront such tendencies, governments and consumer protection agencies have established guidelines and regulations, such as \cite{GDPR1,GDPR2,CCPA}. 
In a nutshell, these documents require from organizations to provide users with ``the right to be forgotten'', i.e., removal of users' data upon request. 
In the simplest scenario, this means removal of the part of a big dataset pertaining to a single user, or a group of users. 
However, the corporate entity might be incentivized to ignore or violate the removal request for a number of reasons. 
First of all, the performance of trained models can degrade after the data removal procedure, resulting in financial losses. 
Besides, removal generally requires to retrain the statistical model, which might be computationally costly. 
While techniques for removing the impact of data points from a model without retraining it have been proposed~\cite{guo2019certified},
their analysis is only tight in simple cases, and lacks generalization guarantees. 
Thus, users might be interested in verifying whether the corporate entity complied with their deletion requests. Ideally, such verification is to be done by a third party (``auditor''), without compromising the privacy of neither users' nor entity's data and trained models.

Our hypothesis testing framework can be used to provide such arbitrage. % of ``the right to be forgotten''.
To this end, we view~$\Prob_0$ as the original dataset and~$\Prob_1$ the dataset after receiving (potentially many) data removal requests (both datasets are assumed to be large, hence modeled by population distributions). The respective population risk minimizers~$\theta_0, \theta_1$ correspond to the model trained with or without the datapoints to be removed. 
Under~$\cH_1$,~\learner{} (i.e., the corporate entity) indeed removed the data, whereas~$\cH_0$ corresponds to the request violation; in both cases,~$\theta^*$ is the {\em actual} model trained by~\learner. The \auditor{}, which can be an external or internal agent in a technological platform, can verify the data removal by examining  the trained model~$\theta^*$ using ``snapshots'' of the two datasets, which corresponds to measuring ``empirical prediction scores'' of~$\theta^*$ on the samples from~$\Prob_0$ and~$\Prob_1$. 
Such verification does not require to provide~\auditor{} with direct access to neither the trained model (i.e.,~$\theta^*$) nor the full datasets~($\Prob_0,\Prob_1$). 
Moreover, as previously discussed, the sample complexity of such testing is way smaller than that of estimating~$\theta^*$. 
In practical terms, this means that \auditor{} will not be able to recover the trained model when running a testing procedure: indeed, the dataset snapshots are sufficient for testing but too small for estimation.

\paragraph{User identification.}

Consider the task of identifying a user whose data has been used to train a predictive model. %, from a snapshot of their data. 
Here, there are~$m$ datasets~$\Prob_1, ..., \Prob_m$, pertaining to~$m$ users of a data platform. 
In a similar vein to the previous example, the \auditor{} must infer which of those~$m$ datasets has been used by the~\learner{} to train the model. 
This can be done by measuring the prediction scores of the trained model on the snapshots of~$m$ datasets.
Note that this application requires to extend the framework to multiple testing; as such extension can be done in a standard way, we omit it here.
%to the datasets of~$m$ users; the task is to define which user's data has been used to learn the model.


\paragraph{\odima{Add a picture describing the arbitrage protocol}}


\paragraph{\odima{Add another application? Maybe sth related to fairness and protected groups...}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MEISAM/ADEL's TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

%While these guidelines seem  necessary to limit the potential adverse impact of AI, it is still not clear how to test for potential violations of these guidelines.
%As a first step towards building tools for this task, we develop a hypothesis testing procedure that verifies the type of data used in the training of a statistical model. Before describing our framework and results in detail, we briefly summarize the problem statement.

The above problem appears naturally in the context of auditing ML platforms for the violation of user privacy, where the auditor suspects that the learner utilizes unauthorized  data points or  features for training their model. 
This problem also can be motivated by ``the right to be forgotten'', enacted by various legislations %such as the General Data Protection Regulation \cite{GDPR1, GDPR2} or the California Consumer Privacy Act \cite{CCPA}. 
(\cite{GDPR1, GDPR2,CCPA}), that grants users the right of deleting their data on request.
%These regulations grant the right of deleting their data to users (data owners).  
%impact a wide range of technological platforms. 
While deleting data from the database is effortless, removing the {\em effect of such data on a trained ML model} can be extremely challenging~\cite{villaronga2018humans}. 
In particular, the {model inversion}  and {membership inference} attacks have demonstrated the possibility of extracting individuals' data by just inspecting the trained ML models~\cite{backes2016membership, dwork2015robust, homer2008resolving, sankararaman2009genomic, veale2018algorithms, salem2018ml, fredrikson2015model, shokri2017membership, ganju2018property, carlini2019secret}. 
%Thus, the right to be forgotten  not only is comprised of removing data from databases, but also includes the removal of the impact of the individuals' data from the trained ML models~\cite{cao2015towards, villaronga2018humans, ginart2019making}. 
% per their request
Consequently, many works developed computationally efficient methodologies for removing the impact of data points from a trained  model~\cite{ginart2019making, baumhauer2020machine, bourtoule2019machine,cao2015towards, golatkar2020forgetting, izzo2020approximate, liu2020learn, schelter8364amnesia, sommer2020towards, xue2016right, guo2019certified}. These works assume the presence of a ``skilled and  honest'' \learner{} that can remove the impact of individuals' data per their requests. However, there are multiple incentives for the learner to avoid the complete removal of data upon request. For example, the performance of trained models can degrade after the data removal procedure, resulting in financial losses. In addition, the data deletion procedure, also known as ``unlearning'',   might be computationally expensive for the learner. %In some cases, this process might involve the complete retraining of the machine learning model from scratch. 
Even when the learner is honest, the unlearning procedure might not completely remove the impact of data points requested to be deleted. For example, the procedure in~\cite{guo2019certified} is accurate for quadratic loss, 
but can be far from optimal in other cases. 
%\end{comment}

In the context of data removal, our problem formulation can be regarded as a methodology for verifying data removal procedures. Namely, $\Prob_0$ can be viewed as the original dataset and $\Prob_1$ as the dataset after receiving (potentially many) data removal requests. The \auditor, which can be an external or internal agent in a technological platform, needs to verify the data removal. %procedure by examining  the training model using samples from the two distributions.  
From this viewpoint, perhaps the work~\cite{sommer2020towards} is the closest to ours. This work requires the backdoor injection  by perturbing the training data of each user so that detecting removal becomes possible later on if needed. This assumption is impractical in scenarios where users cannot perturb their data before sharing with the learner. Moreover, the learner might detect  backdoors and remove them from  data. %Even when the platform does not remove the backdoors, in the presence of many deletion requests, the entire probability distribution may change which cannot be handled by methodologies for verifying single (constant) number of deletion requests.

\end{comment}


\begin{comment}
Instead of working with complex data poisoning or backdoor attacks, to gain theoretical insights on the problem formulated above, we start by rigorously studying the simple case of linear regression. We analyze how many samples from the two distributions~$\Prob_0$ and $\Prob_1$ the auditor needs to make a confident decision. We develop a statistical test with near-optimal sample complexity in this scenario. Then, using the insights from the case of a linear model, we develop testing procedures for the more general setup, and prove performance guarantees for such procedures.
But before that, we state the problem in the language of hypothesis testing, and discuss the arising challenges. 
\end{comment}


\begin{comment}
Newton decrement has been used in contexts different than ours, such as measuring group effects, data poisoning, estimating generalization, and even algorithms for data deletion, to name just a few; see~\cite{koh2019accuracy, jaeckel1972infinitesimal, koh2017understanding, hampel1974influence, guo2019certified, koh2018stronger, beirami2017optimal, wilson2020approximate} and the references therein.
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%is the ones appeared in \cite{sommer2020towards, chen2020machine} 


% For most ML models which aim at minimizing average loss over the training dataset, we need to ensure that there is not a representation disparity for subpopulations. Otherwise, the minority subpopulations which contribute less to the training data will suffer higher test error.


% In what follows, we give a few examples where this technical problem naturally appears. {\color{blue}{To Meisam: Can you add pointers to data deletion from Percy's work? Not sure how much we want to expand these bullets}}
% \odima{no need to expand, and we do need references!} \odima{to ALL: please use the macroes I defined for everybody:} \simo{for Simo}, \adel{Adel}, \meisam{Meisam}.


% \begin{itemize}
%     \item Data deletion (removing some entries or some features for some data points)
%     \item Checking for individuals' privacy violation (in features or data points)
%     \item Using data from a third party vendor/model, Augment their dataset by ML model stealing.
%     \item Fairness: For most ML models which aim at minimizing average loss over the training dataset, we need to ensure that there is not a representation disparity for subpopulations. Otherwise, the minority subpopulations which contribute less to the training data will suffer higher test error.  
% \end{itemize}

%\odima{{\bf TODO:} Extend the discussion, remove half of citations (listing them is not a good idea; maybeput into a dedicated related work section?)}





==> setup.tex <==
\section*{Problem setup \odima{TODO: Mostly remove, but merge the auditor-related discussion to Sec.~\ref{sec:applications} and preserve somewhere the discussion of~\eqref{eq:test_naive}?}}
%\label{sec:setup}

%\vspace{-0.2cm}

%We view the problem through the lens of statistical learning theory.
%Namely, we 
Let~$\ell_z(\theta): \R^d \to \R$ be the loss function used by the~$\learner$ to measure the performance of a candidate model~$\theta \in \R^d$ on the data point~$z \in \cZ$, where~$\cZ$ is the observation space. This function is not assumed to be known to the \auditor{}.
%We focus on supervised learning setup, where~$z = (x,y)$ with~$x \in \R^d$ representing the covariates  (features) and~$y \in \cY$ for some label space~$\cY$,~e.g.,~$\cY = \R$ for regression and~$\cY = \{\pm 1\}$ for binary classification tasks. 
%In many practical situations, one further focuses on {\em generalized linear models} (GLMs), where~$\cY \subset \R$, and the loss takes the form~$\ell_z(\theta) = \phi(x^\top \theta, y)$ for some cost function~$\phi: \R \times \cY \to \R$; this is the case, e.g., in linear regression, robust regression with the Huber loss, logistic regression and support vector machines, and their kernelized versions (when~$d = \infty$).
%\paragraph{General setup.}
With the loss function~$\ell_z(\theta)$ at hand, the learner fits its model by minimizing the loss averaged over the the full dataset which is assumed very large and hence modeled as a distribution~$\Prob$ on~$\cZ$. 
In other words, the learner computes a population risk minimizer~$\theta^*$ according to~$\Prob$,
\[
\theta^* \in \Argmin_{\theta \in \R^d} \left\{ \, L(\tht) := \E [\ell_z(\tht)] \, \right\},
\] 
where the expectation is over the distribution~$\Prob$ of~$z$. 
We assume there are two possibilities for this distribution, namely~$\Prob_0$ and~$\Prob_1$, 
and the \auditor{}'s task is to determine from which of the two distributions~$\theta^*$ actually stems. 
In other words, the task is to distinguish between the two hypotheses
\[
\cH_0: \{\theta^* = \theta_0 \}, \quad 
\cH_1: \{\theta^* = \theta_1 \},
\]
where~$\theta_0$ and~$\theta_1$ are the minimizers of the population risks
$
L_0(\tht) := \E_0[\ell_z(\tht)] 
$ and~$
L_1(\tht) := \E_1[\ell_z(\tht)]
$
corresponding to~$\Prob_0$ and~$\Prob_1$.
To this end, the auditor obtains two samples with i.i.d.~observations
\[
z_1, ..., z_{n_0} \sim \Prob_0, \quad 
\wt z_1, ..., \wt z_{n_1} \sim \Prob_1,
\]
corresponding to ``snapshots'' of the full datasets,

% and has {limited access} to the unknown model~$\theta^*$ through local empirical risk oracles.  
and can evaluate the learned model~$\theta^*$ on both samples by measuring the empirical risks
\begin{equation}
\label{def:emp-risks}
%\textstyle
\wh L_0(\theta) := \frac{1}{n_0}\sum_{i=1}^{n_0} \ell_{z_i}(\theta), \quad
\wh L_1(\theta) := \frac{1}{n_1}\sum_{i=1}^{n_1} \ell_{\wt z_i}(\theta).
\end{equation}
In addition, we assume the auditor is given access to the local second-order information about empirical risks, namely, to their gradient and Hessian at~$\theta^*$. 
\odima{Note that, in principle, the gradients and Hessians can be approximated with arbitrarily high accuracy via finite-difference methods if one is given access to the values of empirical risks in an arbitrarily small neighborhood of~$\theta^*$.}
%in a neighborhood of~$\theta^*$ -- or, equivalently, access to~$\nabla^s \wh L_k(\theta^*)$ for~$s = 0,1,...$ and~$k \in \{0,1\}.$ {\color{blue}{This should be written more rigorously, what should be the size of neighborhood? what does $s=0$ mean? Do you need all $s$? Maybe you first write what derivatives you need and then explain that by finite difference methods this reduces to loss evaluations in arbitrary small neighborhood of the true model }} \odima{Maybe change the flow a bit by putting this as a remark after the non-Gaussian sec.}
Equipped with this information, we are interested in how fast the \auditor{} can achieve reliable conclusion. This can be formalized as the sample complexity, in terms of~$n_0$ and~$n_1$, to guarantee fixed probabilities of error of one or both types. 
To shed more light on this setup, we make a few immediate observations.
% they also shed light on our results which follow next.

% \begin{itemize}
% \item 

First, we aim to minimize the needless disclosure of information to the auditor in what concerns both the learner (by prohibiting full access to the learned model itself) and the data owners (by only allowing sampling rather than full access to~$\Prob_0$ and~$\Prob_1$). 
If the auditor receives full, rather than local, access to both empirical risks, she can in principle learn both models~$\theta_{0}$ and $\theta_1$ by performing empirical risk minimization (ERM). 
One of these models is equal to~$\theta^*$ (if~$L(\cdot)$ is strictly convex) or has the same prediction performance (if~$L(\cdot)$ is convex). Thus, when~$n_0, n_1 \to \infty$, both facets of privacy get compromised, and we are naturally interested in keeping~$n_0, n_1$ as small as possible. 
In this connection, it is quite fortunate that the sample complexity of reliable testing between~$\cH_0$ and~$\cH_1$ turns out to be essentially {\em dimension-independent}: as we establish in Secs.~\ref{sec:gaussian}--\ref{sec:asymp}, this complexity only depends on certain measure of separation between~$\theta_0$ and~$\theta_1$ whenever this separation is larger than a certain threshold that {\em decreases} with the model intrinsic dimension. In contrast, the sample complexity of consistent empirical risk minimization is typically polynomial in~$d$ -- in particular,~$n = \Omega(d)$ is required for constant prediction error in random-design least-squares~(\cite{hsu2012random}). 
%thus, we aitm suggested methodology typically outperforms the naive ERM approach. 
% our testing procedure has guaranteed performance when the sample size is way smaller than~$d$ (which is nes, e.g., to control the prediction error in the simplest case of random-design least-squares). 
%In Sec.~\ref{sec:gaussian}, we investigate this phenomenon for linear models, and in Sec.~\ref{sec:general} we extend the results to more general situations.

%\item
Second, granting auditor access to higher derivatives of~$\wh L_{0}$ and $\wh L_{1}$ at~$\theta^*$ might seem redundant. Indeed, assume, for the moment,
% purpose of this discussion, 
that the optimal population risks~$L_{0}(\theta_0), L_{1}(\theta_1)$ are known. 
One has a natural test that only uses the values~$\wh L_{0}(\theta^*),\wh L_{1}(\theta^*)$ of empirical risks:
%(and no higher derivatives) 
% accept the hypothesis corresponding to
\begin{equation}
\label{eq:test_naive}
  \hat{T} = \ind\big\{ 
\wh L_{0}(\theta^*) - L_0(\theta_0) \geq \wh L_{1}(\theta^*) - L_1(\theta_1)
\big\}.
\tag{$\texttt{\textup{Val}}$}
\end{equation}
This test can also be used when~$L_{0}(\theta_0)$ and~$L_{1}(\theta_1)$ are unknown, but known to be {\em equal}. 
This is the case, e.g., in a well-specified linear model considered in Sec.~\ref{sec:gaussian}.
% \wh T(\theta^*) = 
Under~$\cH_0$, the term~$\wh L_{0}(\theta^*) - L_0(\theta_0) = \wh L_{0}(\theta_0) - L_0(\theta_0)$ randomly fluctuates around zero, whereas the term~$\wh L_{1}(\theta^*) - L_1(\theta_1) = \wh L_{1}(\theta_0) - L_1(\theta_1)$ fluctuates around the excess risk~$L_1(\theta_0)-L_1(\theta_1)$, with amplitude of fluctuations decreasing as~$n_0$ grows. A similar situation occurs under~$\cH_1$. As such, test~\eqref{eq:test_naive} is consistent when~$n_0, n_1 \to \infty$ as long as~$\theta_0$ and~$\theta_1$ are separated in terms of excess risks with respect to~$\Prob_0$ and~$\Prob_1$. Surprisingly, this test turns out to be suboptimal: we show that one can achieve better results by exploiting the second-order information and using the {\em Newton decrements} of empirical risks instead of their values.
For linear models (see Sec.~\ref{sec:gaussian}), this corresponds to reducing the magnitude of the noise by projecting the vector of residuals onto the signal subspace before measuring its norm. 


%which reduces the magnitude of fluctuations. 
% in the form of the Newton decrements of~$\wh L_{0}$ and~$\wh L_{1}$~(\cite{nesterov2013introductory}). 
%In the case of a linear model, this has a simple interpretation: it corresponds to projecting the residuals to the signal space, which reduces the variance of the chi-squared statistic (see Sec.~\ref{sec:gaussian}).
% i.e., (the squared) local norm of the gradient. In the case of a linear model, the 

% in a sense, the fluctuations can be reduced by projecting the noise to the signal space, which amounts to comparing the 
% statistic that encapsulates the gradients and Hessians of empirical risks. 
% \odima{Here is too early for this discussion in the text. All these are good to discuss after the result.}
% {\color{red} We can also talk about other tests. The more natural gradient test 
% \[
%   \hat{T}_g = \ind\big\{ 
% \nabla\wh L_{0}(\theta^*) - \nabla L_0(\theta_0) \geq \nabla\wh L_{1}(\theta^*) - \nabla L_1(\theta_1)
% \big\},
% \]
% That is sub-optimal in terms of the separation required. Or the test that mimicks an oracle having access to both $\theta_0$ and $\theta_1$ given by 
% \[
% \hat{T}_o = \ind\big\{ 
% \wh L_{0}(\theta^*) + \hat{L}_1(\hat{\theta}_1+\hat{\theta}_0 - \theta^*)  \geq \wh L_{1}(\theta^*) + \hat{L}_0(\hat{\theta}_1+\hat{\theta}_0 - \theta^*)
% \big\}.
% \]
% The last test is sub-optimal since it only performs well when parameter estimation is possible and hence requires a stronger separation. I am planning to compare all of these tests in my simulations.
% }

% Our testing procedures do not use higher derivatives of the empirical risks. 

In what follows, we first study the simple case of a well-specified linear model to showcase our methodology. 
We then consider a more realistic setup involving generalized linear models in Sec.~\ref{sec:glm}. 

% In what follows, we consider the simple case of a well-specified linear model. We construct a test based on the properly adjusted squared loss statistic, and prove that this test is statistically near-optimal. After that we extend the approach to the non-linear case using the Newton decrement. 
% \end{itemize}


==> simul-old.tex <==
\section{Numerical experiments}
\label{sec:simul}
%\vspace{-0.2cm}
%###########################################

\odima{\bf Write this properly.}

We compare the empirical performance of several tests in the case of a well-specified linear model:
\begin{itemize}
\item[(a)] 
our proposed test~\eqref{eq:test_1}; 
\item[(b)] the test~\eqref{eq:test_naive} based on the values of empirical risks;
\item[(c)] the gradient norm test~\eqref{eq:test_grad} (cf.~Rem.~\ref{rem:gradient-test}); 
\item[(d)] the oracle test that corresponds to the (suboptimal) likelihood-ratio oracle test~$T_{LR}$ arising in the proof of Theorem~\ref{th:lower-gaussian} (cf.~\eqref{eq:test-oracle} in Appendix~\ref{app:lower}):
\[
\mathbf{1}\{ \| Y - X\theta^*\|^2 + \| \tilde{Y} - \tilde{X} ({\theta}_0 + {\theta}_1 - \theta^*)\|^2 \leq \| Y - X({\theta}_0 + {\theta}_1 - \theta^*)\|^2 + \| \tilde{Y} - \tilde{X} \theta^{*}\|^2 \}.
\]
\item[(e)] the plug-in test that ``mimics'' the oracle above by replacing~$\theta_0,\theta_1$ with their least-squares estimates~$\wh \theta_0,\wh \theta_1$:
\[
\mathbf{1}\{ \| Y - X\theta^*\|^2 + \| \tilde{Y} - \tilde{X} (\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 \leq \| Y - X(\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 + \| \tilde{Y} - \tilde{X} \theta^{*}\|^2 \}.
\]
\end{itemize}
% \begin{itemize}
%     \item The loss test as described in \eqref{eq:test_naive}.
%     \item The gradient test as given in \eqref{eq:test_grad}.
%     \item The plug-in estimator that mimics the oracle (cf. Proof of Theorem \ref{th:lower-gaussian}) by estimating $\theta_0$ and $\theta_1$ and that is given by:
%     \[
%      \hat{T} = \mathbf{1}\{ \| y - X\theta^*\|^2 + \| \tilde{y} - \tilde{X} (\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 \leq \| y - X(\hat{\theta}_0 + \hat{\theta}_1 - \theta^*)\|^2 + \| \tilde{y} - \tilde{X} \theta^{*}\|^2 \}.
%      \]
%     \item And finally, our test \eqref{eq:test_1}.
% \end{itemize}

%\vspace{-0.2cm}

In our simulations, we set~$n_0 = n_1 = 100$.
We take diagonal~$\bSigma_0,~\bSigma_1 \in \R^{100 \times 100}$ with rank~$r\in\{40,80\}$; the elements on the diagonal of~$\bSigma_0$ are given by~$\lambda_1 = \dots = \lambda_{15} = 1$ and~$\lambda_{16} = \dots = \lambda_{30} = \kappa$ with~$\kappa \geq 1$ specified further on; the diagonal of~$\bSigma_1$ is a random permutation of that of~$\bSigma_0$. 
For each value of~$\kappa \in \{10,50\}$, simulation is repeated~$50000$ times; we present the probability of error for the  tests (a-e) in Figure~\ref{fig:comparison} and \ref{fig:comparison2}. Overall, numerical experiments confirm our theoretical predictions. Our test~\eqref{eq:test_1} has the best performance regardless of~$\kappa$ and $\rank$ although its performance decreases as the $\rank$ grows while the performance of the oracle stays the same (which is expected). On the one hand, in the large rank regime, while the plug-in test fails as estimation of $\theta_0$ and $\theta_1$ is costly, the loss test is almost as good as our test since the projection step is trivial. On the other hand, as the rank gets smaller, the plug-in test behaves better and the loss test loses its efficiency. Notice also that the gradient test performs poorly as~$\kappa$ grows. 


%\vspace{-0.3cm}
\begin{figure}[ht]
\centering
\hspace{-.cm}
\begin{subfigure}{}
  \centering
 \includegraphics[width=.8\linewidth]{arXiv-v1/exp_r80_k10.pdf}
%   \includegraphics[width=.3\textwidth]{figs/kappa_one_legend_up.pdf}
  \label{fig:sub1}
\end{subfigure}
\centering
\begin{subfigure}{}
  \centering
% \includegraphics[width=.3\linewidth]{figs/kappa_ten_legendless.eps}
%   \includegraphics[width=.3\textwidth]{figs/kappa_ten_legendless.pdf}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{}
  \centering
% \includegraphics[width=.3\linewidth]{figs/kappa_fifty_legendless.eps}
%   \includegraphics[width=.3\textwidth]{figs/kappa_fifty_legendless.pdf}
  \label{fig:sub3}
\end{subfigure}
%\vspace{-0.4cm}
\caption{Average testing error over $50000$ runs of the experiment with $\rank = 80$ and $\kappa = 10$. The plot is with respect to $n\Delta^2$.}
\label{fig:comparison}
\end{figure}

\begin{figure}[ht]
\centering
\hspace{-.cm}
\begin{subfigure}{}
  \centering
 \includegraphics[width=.8\linewidth]{arXiv-v1/exp_r40_k50.pdf}
%   \includegraphics[width=.3\textwidth]{figs/kappa_one_legend_up.pdf}
  \label{fig:sub1}
\end{subfigure}
\centering

%\vspace{-0.4cm}
\caption{Average testing error over $50000$ runs of the experiment with $\rank = 40$ and $\kappa = 50$. The plot is with respect to $n\Delta^2$.}
\label{fig:comparison2}
\end{figure}
% \simo{We can now move the content below to intro and remove Broader impact
% \section*{Broader Impact}
% In addition to the applications in checking the potential violation of individuals' privacy and verifying the data removal procedures,   the methodologies and  theoretical insights in this work can be used for other possible auditing purposes. For example, in the context of fair machine learning~\cite{datta2015automated, sweeney2013discrimination, bolukbasi2016man, machinebias2016}, we need to ensure that there is not a representation disparity for sub-populations. Otherwise, the minority sub-populations which contribute less to the training data will suffer higher test error. In this context, the auditor is interested in testing whether the training data has equal representation of sub-populations. Such an auditor can be viewed as the basic building block of the \textit{multiparty computation framework} proposed in \cite{jagielski2018differentially, veale2017fairer, kilbertus2018blind}. }

